What Do Deep CNNs Learn About Objects?

Deep convolutional neural networks learn extremely powerful image representations, yet most of that power is hidden in the millions of deep-layer parameters. What exactly do these parameters represent? Recent work has started to analyse CNN representations, finding that, e.g., they are invariant to some 2D transformations Fischer et al. (2014), but are confused by particular types of image noise Nguyen et al. (2014). In this work, we delve deeper and ask: how invariant are CNNs to object-class variations caused by 3D shape, pose, and photorealism?

==> datageneration.tex <==
\section{Virtual data generation}
\label{datageneration}

Data generation method for our model is quite similar with that used in~\cite{BMVC}. The main differences are: 1) they used only 2 CAD models per category while we use more models to cover the intra-class variations; 2) we add real-image background and texture to virtual images in an attempt to make them more realistic.

The CAD models are downloaded from 3D Warehouse by searching for the name of 20 object categories in the PASCAL Dataset. For each category, about 25 models were downloaded. Original poses of some of the CAD models can be arbitrary, for example, upside-down chairs or slanted cars. We adjust the CAD models's pose manually to 3-4 poses that best represent intra-class pose variance for PASCAL objects. Then for each model pose we generate 1-2 virtual images to form a virtual training dataset. The final number of images in the virtual training dataset is 2,000, with 100 positive instance per each of 20 categories.

To investigate the importance of realistic backgrounds and object textures, we downloaded some real images for each category. When generating virtual images, we randomly select a background image from this pool to project to the image plane and a texture image to map onto the CAD model. We also tried different generation settings as shown in Table \ref{tab:datageneration}.

\begin{table*}[ht]

\begin{center}
\begin{tabular}{|l||c|c|c|c|c|c|}
\hline
NO. &\textbf {R-R} & \textbf{W-R}&\textbf{W-UG}  &\textbf{R-UG}&\textbf{RG-UG}&\textbf{RG-R}\\ 
\hline
BG & Real&White & White &Real&Real Gray&Real Gray\\
\hline
TX &Real & Real&Uni Gray&Uni Gray&Uni Gray&Real\\
\hline

Sample& \includegraphics[width=0.5in]{real_real.jpg}
&\includegraphics[width=0.5in]{white_real.jpg}
& \includegraphics[width=0.5in]{white_gray.jpg}
&\includegraphics[width=0.5in]{real_gray.jpg}
&\includegraphics[width=0.5in]{realgray_gray.jpg}
&\includegraphics[width=0.5in]{realgray_real.jpg}\\

\hline

\end{tabular}
\end{center}
\caption{Samples for different configuration of data generation. For background(BG), we have tried real images, white scene, and real gray images; and two types of texture, ie. real image texture and uniform gray.}
\label{tab:datageneration}


\end{table*}



==> images/approach.tex <==
\section{Virtual Data Generation}

Data generation method for our model is quite similar with that used in~\cite{bmvc}. The main differences are: 1) they used only 2 CAD models per category while we use more models to cover the intra-class variations; 2) we add real-image background and texture to virtual images in an attempt to make them more realistic.

The CAD models are downloaded from 3D Warehouse by searching for the name of 20 object categories in the PASCAL Dataset. For each category, about 25 models were downloaded. Original poses of some of the CAD models can be arbitrary, for example, upside-down chairs or slanted cars. We adjust the CAD models's pose manually to 3-4 poses that best represent intra-class pose variance for PASCAL objects. Then for each model pose we generate 1-2 virtual images to form a virtual training dataset. The final number of images in the virtual training dataset is 2,000, with 100 positive instance per each of 20 categories. \kate{how do we generate 2 images, what changes? and why not always 2?}

To investigate the importance of realistic backgrounds and object textures, we downloaded some real images for each category. When generating virtual images, we randomly select a background image from this pool to project to the image plane and a texture image to map onto the CAD model. We also tried different generation settings as shown in Table??.

\kate{[Insert a Table to clarify]}

\section{Exploring the Invariances of the CNN}

Before training our VCNN model, we design a series of experiments to evaluate how deviation of various image formation factors such as the color, texture, background and pose of an object from those found in real images influence CNN model's performance. Using computer graphics techqnies we can easily the factors mentioned above to investigate the CNN's invariance.

For each experiment below, we training only the output layer of the network, using deep features pre-trained on real images ad inputs.	

\subsection{Color, texture, background}

Empirically, color, textures, shape and background information are all critical to CNN. Because the convolutional layers are directly applied to the raw pixels of an image, local patterns and intensity are decisive to which neural unit will fire. It is therefore unclear whether the gap between realistic images and non-photorealistic virtual images, which lack realistic color, textures, and background information will cause the CNN to fail to produce a useful representation.

To get better training configuration for the VCNN, we have tried a batch of experiment configurations for background, color and texture for the virtual images. To better align to the real images, the features extracted by RCNN for the following experiments are fine-tuned by PASCAL 2007 train+val datasets. 

\kate{	[Figure to insert: pipeline]}
\kate{	[Table to insert:]}

\cite{bmvc} showed that for training a HOG template model on virtual data rendered from CAD models, rendering natural backgrounds and textures is not needed, white backgrounds and uniform gray textures can be used with similar results. Their claim is that a discriminative HOG-based classifier basically learns the ``outlines'' of the object shape, and discards everything else. The HOG model can arguably even learn from line drawings of the objects, although this remains to be proven experimentally.

Now, would that be the case for deep CNN models? Can you train a classifier using deep features on line drawings? The answer would seem to be no, because the deep layers capture not just shape outlines, but complex mid-level features such as faces, object parts and other patterns. However, we can show experimentally that again, learning from white background and uniform gray texture achieves similar performance as learning from natural backgrounds and realistic textures. At least this is the case when training only the output layer of the network, using deep features pre-trained on real images.	

\kate{move this to result section, instead explain the generated backgounds etc}


From the results of VCNN pipelines, we find that if the contour of the whole object is more distinguished from the background, the mAP is likely to be higher though from the visualization of pool5 units shows that many units are fired on the parts of an object. 

\subsection{Pose Variation}

From different viewpoints, the same object may have absolutely different presentations. Many works 
%[cite http://cvgl.stanford.edu/papers/3D%20generic%20object%20categorization_iccv07.pdf ] 
have focused on studying the effect of pose in detection tasks. Thanks to the pooling layers in the CNN, the deep features are kind of invariant to rotation and perspective transformation. But when the pictures of a certain object are taken from totally different views or the object is deformable, they could be totally different to computer. Take horses for example, the contour of prominent side-view horse is different from the horses from front-view.

In this experiment, we select 12 categories from PASCAL, for which the front-view and side-view are easy to distinguish. For other categories such as bottle and table, it's hard to define the side-view and front-view.

We split the training data for these 12 categories to prominent side-way and front-view, as showed by [insert a figure]. We have carried out a set of experiments to study the effects of pose to RCNN. The experiments are showed in table [insert a table]. It shows that removing a certain pose from the SVM layer of RCNN model fine-tuned with both front-view images and side-view images, the mAP will only drop by 1 or 2 points. If RCNN model is only fine-tuned by images with front-view objects, the mAP will drop by 2 points if the SVM is still trained on both views, but will drop by 5 points if the SVM is also trained with only front-view objects.  

The RCNN model is pre-trained on 1.2m class-labeled images from Image-net and 17 categories from PASCAL are already included in Image-net. The fact that the RCNN model has already seen both views while pre-training may partly explain why there is only a little drop when removing one view. 

We have proposed an assumption that the deep features are invariant to pose by parts. Take two absolute different view-points of cars for example, one is absolute front-view and from this view, only the headlamp, front cover and cab are visible; the other is absolute side-view and only doors, wheels and windows are visible .If a CNN model is not pre-trained on cars and not fine-tuned on images with both views, it will take the cars with these two different views for different categories. The visualization of pool5 features shows that wheels are actually a distinguished part of a car and many neurons are fired on wheels. So it will be very interesting when it comes to an intra-view cars from which we can see a part of wheels, doors, windows and maybe headlamp. When the RCNN model is training only on the intro-view cars, it will probably still can find out the absolute side-view cars for they both have wheels and doors to fire the correspondent neurons.

From this point, when training our VCNN model, we fix the CAD models to 3-4 prominent poses, and rotate the 3D model by a random angle from 0 to 20 degrees in each of the three axes.

\subsection{Variation in 3D Models}


In \cite{bmvc}, only 2 models per category are used to align the Office dataset because the intra-class variation of Office dataset is small. But there are more refined categories for a certain categories in PASCAL. The authors of~\cite{xiang2014beyond} used around 9 CAD models to align the PASCAL detection dataset. But from our experiments, we find that the mAP will decrease by about 5.5 points from 28.9\% to 23.53\% when using only a half number of the 3D models described in section 2.1. And it requires more 3D models for the deformable categories in PASCAL.

\kate{NEED TO PUT ALL ABOVE results NuMBers in tABLES}

%%%%%%%%%%%%%%%%%%%
\section{ Experiments}

Detectors based on deep CNNs, including OverFeat and RCNN, need a large quantity of real training images and a lot of manual annotation work. There are only 20 categories in PASCAL and 200 categories in the ImageNet detection dataset. For many novel categories, the training data is limited. 

\subsection{Data acquisition}

Through the detailed descriptions above and dense experiments on finding out what really matters to train a VCNN, we finally choose the virtual images with real-images background and real-images texture.  We find it's important to use this configuration because: 1). When the CNN learns distinguished features for one category, the information from background is also very important. From previous works on image classification, the CNN will mistake the truck in the snow for snow plough because the background for the snow plough category is critical. 2). Textures on object are also important because the CNN is operated on the raw pixels. 

Although the virtual dataset with white background and uniform gray texture can get a comparable mAP with virtual dataset with real-image background and real-image texture, the visualization of the positive training data shows that the white patch around the objects makes it harder to sample negative training data, under the schema of selective search.

\subsection{Results of experiments on color, texture, background}

The experiments indicate that the mAP is determined by how distinguished the object is from the background. When using the uniform gray texture and the white background, the mAP-30.14\% is comparable to the mAP-28.9\% from VCNN trained by virtual images with real-image background and real-image texture. And when using the non-colored real-gray background with colored real image texture on the target objects, the mAP is 31.18\%, 6-9 points higher than the performance of VCNN trained on virtual images with real-image background and uniform gray texture and VCNN trained on virtual images with real-gray background and uniform gray texture, in which the foreground images are not quite distinguished from the background.



\subsection{Results of Final VCNN Configuration}
\kate{not entirely happy with this title}

\kate{refer to results figure}
Our model obtains a mAP of 27.05\% on PASCAL detection test dataset with 2k virtual images. The pipeline of our model is similar to RCNN, with region proposal by selective search, similar CNN architecture designed by Krizhevsky et al [cite], and supervised pre-training. The difference is that, instead of depending on the manually annotated PASCAL trainval dataset, we use only 2k virtual images to fine-tune the pre-trained CNN and use the features extracted by the fine-tuned CNN to train the SVM. We strongly recommend our paper readers to refer RCNN for more details.

At test time, we run selective search on the test images to extracted around 2k region proposals and forward propagate each warped region proposal through VCNN to extract the feature using the Caffe [cite] implementation of CNN. Then using the corresponding SVM to score the 4096-dimensional feature vector. Then apply non-maximum suppression to all the scored proposals to reject a proposal if it has an IoU overlap with a higher score.

\kate{[Insert a pipeline here to show how it works]}
      
\kate{move to results} 
It’s often the truth that there are no annotated realistic images for a novel category.   When VCNN model is only pre-trained on Image-net, the mAP is 23.32\%.When the network is fine-tuned by Pascal trainval datasets, the AP goes to 28.9\%; when the network is fine-tuned on Image-net detection dataset with 200 categories, the AP is 27.24\%. 


\begin{table}[th]
\centering
\begin{tabular}{|l|l|l|c|}
\hline
Pre-train & Finetuning & SVM-Training & mAP \\ \hline
Imagenet 1.2m &
None  &
Virtual & 
23.32 \\ \hline
Imagenet 1.2m  &
Pascal  &
Virtual  &
28.9 \\ \hline
Imagenet 1.2m   &
Imagenet 200 &
Virtual &
27.24 \\ \hline
Imagenet 1.2m  &
virtual &
Virtual &
27.05 \\ \hline

\end{tabular}
\vspace{0.1in}
\caption{Effect of finetuning.}
\label{tab:nets}
\end{table}

We have also designed a set of experiments to simulate the situation that the number of realistic images is limited. Basically, for every category, we will randomly select 20(10, 5) positive training images to form datasets $R_{20}$ ($R_{10}$, $R_{5}$). The sizes of final datasets are 276(120, 73) because there are some images which contain two or more positive data. The size of virtual datasets (noted as $V_{2k}$) is still 2000. We use dataset $R_{x}$ (x=20,10,5) to train RCNN model, $R_{x}$+$V_{2k}$ to train our VCNN model, and $R_{x}$+$V_{2k}$ to train the Fast-Ada model. Due to the training data for RCNN is limited, the RCNN is only pre-trained on Image-net and not fine-tuned. The VCNN model is pre-trained on Image-net and fine-tuned by $V_{2k}$.

The result shows that when the number of training data is limited, VCNN will perform better than traditional RCNN for the lack of training data. The VCNN will also perform better than the Fast Adaptation method described in \cite{bmvc}.
 Refer to Table~\ref{tab:nets} and explain!



\begin{figure}[t]
\begin{center}
%   \includegraphics[width=\linewidth]{mainresult.png}
\end{center}
   \caption{\kate{TODO Comparison with RCNN and White-HOG method\cite{bmvc}}}
\label{fig:main}
\end{figure}



==> related.tex <==
\section{Related Work}
\label{related}

\noindent\textbf{Object Detection.}
``Flat'' hand-designed representations (HOG, SIFT, etc.) have dominated the object detection literature due to their considerable invariance to noise such as brightness, contrast and small translations. In combination with discriminative classifiers such as linear SVM, exemplar-based~\citep{exemplarsvm} or latent SVM~\citep{dpm}, they had proved powerful for learning to localize the global outline of an object. 
%Decorrelation of HOG features via Linear Discriminant Analysis was proposed as Whitened HOG~\cite{who} to avoid costly SVM training while achieving comparable performance.
More recently, convolutional neural networks~\citep{lecun89} have overtaken flat features as clear front-runners in many image understanding tasks, including object detection. 
CNNs learn layered features starting with familiar pooled edges in the first layer, and progressing to more and more complex patterns with increasing spatial support. Extensions to detection have included sliding-window CNN~\citep{Overfeat} and Regions-CNN (RCNN)~\citep{RCNN}.

\noindent\textbf{Understanding Deep CNNs.}
There has been increasing interest in understanding the information encoded by the highly nonlinear deep layers. \citet{zeiler-arxiv-2013} reversed the computation to find image patches that most highly activate an isolated neuron. 
A detailed study of what happens when one transfers network layers from one dataset to another was presented by \citet{yosinskiNIPS14}. 
\citet{mahendran14arXiv} reconstruct an image from one layer's activations,
using image priors to recover the natural statistics removed by the network filters. Their visualizations confirm that a progressively more invariant and abstract representation of the image is formed by successive layers, but do not analyse the nature of the invariances.
Invariance to simple 2D transformations (reflection, in-plane rotation) was explored by \citet{lenc14arXiv}. In this paper, we study more complex invariances by ``deconstructing'' the image into 3D shape, texture, and other factors, and seeing which specific combinations result in representations discriminant of object categories.

\noindent\textbf{Use of Synthetic Data.}
In the early days of computer vision, 3D models were used as the primary source of information to build object models (e.g.,~\citet{nevatia77}).
More recently, \citet{stark_bmvc10,liebelt_cvpr10,sun_cvpr09}
 used 3D CAD models as their only source of labeled data, but limited their work to a few categories like cars and motorcycles. \cite{pinto2011comparing} utilized synthetic data to probe invariances for features like SIFT, SLF, etc. 
In this paper, we generate training data from crowdsourced 3D CAD models, which  can be noisy and low-quality, but are free and available for many categories. We evaluate our approach on all 20 categories in the PASCAL VOC2007 dataset, which is much larger and more realistic than previous benchmarks.
Previous works designed special features for matching synthetic 3D object models to real image data (\citet{liebelt_cvpr08}), or used HOG features and linear SVMs (\citet{BMVC}). We employ more powerful deep convolutional images features and demonstrate their advantage by directy comparing to \citet{BMVC}.
\cite{xiang_wacv14} use CAD models and show results of both 2D detection and pose estimation, but train multi-view detectors not directly on 3D models but on real images labeled with pose.
We avoid expensive manual bounding box annotation, and show results with minimum or no real image labels.
Finally, several approaches had used synthetic training data for tasks other than object detection, for example, \citet{jaderberg14arXiv} recently proposed a synthetic text generation engine to perform text recognition in natural scenes. 

%The majority of other work on utilizing 3D models focused not on detection but on predicting the 3D pose or viewpoint of an object in 2D test images~\cite{liebelt_cvpr10,sun_cvpr09,stark_bmvc10,xiang_wacv14,pepik_cvpr12}, or on categorizing an object from an arbitrary novel viewpoint~\cite{savarese_eccv08}.
%We focus solely on bounding box object detection in 2D real images, and propose a method to build such detectors directly from non-photorealistic CAD models.





==> vcnn.tex <==

\section{Virtual Convolutional Neural Network for Object Detection}
\label{vcnn}
To summarize the conclusions from the previous section, we found that CNNs learn a significant amount of invariance to texture, color and pose, if trained (or fine-tuned) on the same task. If not trained on the task, however, the degree of invariance is lower. Therefore, when learning a detection model for a new category with no or limited labeled real data available, it is preferable to simulate these factors in the synthetic data.

Based on these findings, we propose an approach for using CNNs with CAD-generated virtual images, which we call the Virtual CNN (VCNN).
% for generating synthetic data for use with CNNs, the Virtual CNN. 
Our configuration uses all available 3D models and views, and selects a natural image background and real color image texture for each generated image (\textbf{RR-RR} in Table~\ref{tab:color}. We also propose to fine-tune the layers on the virtual data. 
Our VCNN model is similar to RCNN, with region proposals by selective search and supervised pre-training on ILSVRC. The difference is that, instead of depending on manually annotated real images, we use only the virtual images to fine-tune the pre-trained CNN, and use the features extracted by the fine-tuned VCNN to train the SVM detectors. 

%textbf{Data acquisition}
%
%Through the detailed descriptions above and dense experiments on finding out what really matters to train a VCNN, we finally choose the virtual images with real-images background and real-images texture.  


%The advantages of this configuration are as follows: 1) When the CNN learns distinguished features for one category, the information from background is also very important. From previous works on image classification, the CNN may mistake the truck in the snow for snow plough because the background for the snow plough category is critical. 2). Textures on object are also important because the CNN is operated on the raw pixels. 

We note that there may be other advantages to using realistic backgrounds. Visualizations of the positive training data show that white background around the objects makes it harder to sample negative training data via selective search, as most of the interesting regions are on the object.

%\subsection{Experiments}

%Our model obtains a mAP of 27.05\% on PASCAL detection test dataset with 2k virtual images. 
%At test time, we run selective search on the test images to extracted around 2k region proposals and forward propagate each warped region proposal through VCNN to extract the feature using the Caffe [cite] implementation of CNN. Then using the corresponding SVM to score the 4096-dimensional feature vector. Then apply non-maximum suppression to all the scored proposals to reject a proposal if it has an IoU overlap with a higher score.

%It is often the truth that there are no annotated realistic images for a novel category.   When VCNN model is only pre-trained on Image-net, the mAP is 22.05\%.When the network is fine-tuned by Pascal trainval datasets, the AP goes to 28.9\%; when the network is fine-tuned on Image-net detection dataset with 200 categories, the AP is 27.24\%. 

%\begin{table}[th]
%\centering
%\begin{tabular}{|l|l|l|c|}
%\hline
%Pre-train & Finetuning & SVM-Training & mAP \\ \hline
%Imagenet 1.2m &
%None  &
%Virtual & 
%22.05\\ \hline
%Imagenet 1.2m  &
%Pascal  &
%Virtual  &
%28.9 \\ \hline
%Imagenet 1.2m   &
%Imagenet 200 &
%Virtual &
%27.24 \\ \hline
%Imagenet 1.2m  &
%virtual &
%Virtual &
%27.05 \\ \hline
%
%\end{tabular}
%\vspace{0.1in}
%\caption{Effect of finetuning.}
%\label{tab:nets}
%\end{table}

\noindent\textbf{Learning novel categories.}
We present a set of experiments to simulate the situation where the number of labeled real images for a novel category is limited or zero. For every category, we randomly select 20 (10, 5) positive training images to form datasets $R_{20}$ ($R_{10}$, $R_{5}$). The sizes of final datasets are 276 (120, 73); note that there are some images which contain two or more positive bounding boxes. The size of the virtual dataset (noted as $V_{2k}$) is always 2000. Our VCNN is pre-trained on Imagenet ILSVRC (IMAGENET network) and fine-tuned on $V_{2k}$, then the SVMs are trained on both  $R_{x}$+$V_{2k}$.
We compare the two best configurations from Table~\ref{tab:color}, \textbf{RR-RR} and \textbf{RG-RR}. 

\noindent\textbf{Baselines.} We use datasets $R_{x}$ ($x=20,10,5$) to train the RCNN model, and $R_{x}$+$V_{2k}$ to train the Fast Adaptation method described in \cite{BMVC}. %Because we assume that real training data for RCNN is limited, 
The RCNN is pre-trained on Imagenet ILSVRC, however it is not fine-tuned on detection on $R_{5}$ and $R_{10}$ as data is very limited. 
%For comparison, we also propose a baseline in which the synthetic image dataset is \textbf{RG-RR}.% shown by green line in Figure \ref{results}.



%\kate{mention W-BG baseline}

\noindent\textbf{Results.} The results in Figure~\ref{results} show that when the number of real training images is limited, VCNN will perform better than traditional RCNN. The VCNN also significantly outperfoms the Fast-Adapt method, which is based on HOG features. We also confirm that our proposed \textbf{RR-RR} data synthesis methodology is better than not simulating background or texture. In partcular, fine-tuning on virtual \textbf{RR-RR} data boosts mAP from 18.9\% (Table~\ref{tab:color}) to 22\% without using any real training examples, and to 28\% with 5 real images per category, a 10\% absolute improvement over RCNN. We also notice that the results for \textbf{RG-RR} are much lower than \textbf{RR-RR}, which is not very surprising. Unlike \textbf{RR-RR}, \textbf{RG-RR} with selective search generates many sub-regions without color, and using these regions to fine-tune likely decreases the CNN's ability to recognize realistic color objects.

Note that the VCNN trained with 10 real images per category (200 total) is also using the approximately 900 real images of texture and background. However, this is still much fewer than the 15588 annotated bounding boxes in the PASCAL training set, and much easier to collect as only the texture images (about 130) need bounding box annotation. Yet the obtained 31\% mAP is comparable to the 33\% mAP achieved by the DPM (without context rescoring) trained on the full dataset. This speaks to the power of transferring deep representations and suggests that synthetic CAD data is a promising way to avoid tedious annotation for novel categories.

%9,963 total annotated images in pascal

\begin{figure}
\centering
\includegraphics[width=0.65\linewidth]{images/2.png}
\caption{Detection results of the proposed VCNN on PASCAL. When the real annotated images are limited or not available, eg. for a novel category, VCNN performs much better than RCNN and the Fast Adaptation method.}%\kate{fix zero-ex point for FastAdapt}}
\label{results}
\end{figure}


